Relating Reversible Petri Nets and Reversible Event Structures, categorically

Causal nets (CNs) are Petri nets where causal dependencies are modelled via inhibitor arcs. They play the role of occurrence nets when representing the behaviour of a concurrent and distributed system, even when reversibility is considered. In this paper we extend CNs to account also for asymmetric conflicts and study (i) how this kind of nets, and their reversible versions, can be turned into a category; and (ii) their relation with the categories of reversible asymmetric event structures.

==> contributions.tex <==
% To the best of our knowledge the attempt to relate reversible event structures
% and nets has been done in~\cite{lics}.
%
% The notion of (pre) asymmetric causal net differs from the one of (pre) causal
% net proposed in~\cite{lics} as there forward symmetric conflicts are modelled
% via shared places, whereas here we have pursued the idea that symmetric
% conflicts are represented using asymmetric ones.
% %
% \racn{s} are then obtained by adding reversibility to pre \acn{s}.

% One may wonder, focussing on nets, if we pursue the so called \emph{individual
% token philosophy} or the \emph{collective token philosophy}, as devised
% in~\cite{robindividual}. In the individual token philosophy each place can be
% marked in an \emph{unique} way, whereas in the collective one there may be
% several manners to put a token in a place. If we focus on the forward flow
% only our nets adhere to the individual token philosophy, though asymmetric
% conflicts suggest that the \emph{past} of the transition putting the token in
% a given place may be not unique.
% %
% If we consider also the reversing flow things are not so easy to put apart,
% especially when considering out-of-causal order reversibility, as a forward
% transition may be executed only because some reversing transition has been
% executed.
% %
% The settle the question, probably a different definition for the individual
% token philosophy has to be sought maybe focussing on the forward dependencies
% of the pre asymmetric causal net in the \racn{} rather than considering the
% whole \racn.
%
To the best of our knowledge, the only previous attempt to relate reversible event
structures and nets is in~\cite{lics}.
%
In contrast to the (pre) causal nets proposed in~\cite{lics}, the notion of
(pre) asymmetric causal net considers forward symmetric conflicts represented
by asymmetric ones, rather than via shared places.
%
As a result, \racn{s} are obtained from pre \acn{s} by incorporating reversibility.


Regarding the philosophy behind our nets, it may be asked whether we adhere to
the \emph{individual token philosophy} or the \emph{collective token
philosophy}, as defined in\cite{robindividual}. In the individual token
philosophy, each place can be uniquely marked, whereas in the collective token
philosophy, there can be multiple ways to place a token in a given place.
%
If we only consider the forward flow of our nets, they adhere to the
individual token philosophy. However, asymmetric conflicts suggest that the
\emph{past} of the transition putting a token in a given place may not be
unique.
%
Moreover, when considering the reversing flow, things become more complex,
particularly with out-of-causal order reversibility, as a forward transition
may only be executed because some reversing transition has been
executed.
%
To settle this question, it may be necessary to seek a different definition
for the individual token philosophy, perhaps by focusing on the forward
dependencies of the pre-asymmetric causal net in the \racn{}, rather than
considering the entire \racn.


==> pezzo-prodotto.tex <==
% here below the starting of the construction I believed we had

The category $\mathbf{RACN}$ ha also products. 

\begin{prop}\label{de:racn-prod}
 Let $\resarcn{V}{\bwdset{0}}{0} = (S_0, T_0, F_0, I_0, \mathsf{m}_0)$ and 
 $\resarcn{V}{\bwdset{1}}{1} = (S_1, T_1, F_1, I_1, \mathsf{m}_1)$ be two \racn{s}. Then 
 $\resarcn{V}{\bwdset{0}}{0} \times \resarcn{V}{\bwdset{1}}{1} = (S, T, F, I, \mathsf{m})$ where
 \begin{itemize}
  \item $S = \setenum{\ast}\times S_0 \cup S_1\times\setenum{\ast} \cup \setcomp{(\ast,(t_0,t_1))}{t_i\in T_i} 
        \cup \setcomp{((t_0,t_1),\ast)}{t_i\in T_i}$;
  \item $T = \setenum{\ast}\times T_0 \cup T_1\times\setenum{\ast}\cup \setcomp{(t_0,t_1))}{t_i\in T_i}$;  
  \item $\forall (a,b)\in S\cup T,\ \forall (c,d)\in S\cup T.$ $((a,b),(c,d))\in F$ then either
        \begin{itemize}
         \item if $a = \ast$ and $c = \ast$ then $(b,d)\in F_0$,
         \item if $b = \ast$ and $d = \ast$ then $(a,c)\in F_1$, and
         \item if $a = \ast$ and $b = (s_0,s_1)$ then $(s_0,c)\in F_0$ and $(s_1,d)\in F_1$, and
         \item if $c = \ast$ and $d = (s_0,s_1)$ then $(a,s_0)\in F_0$ and $(b,s_1)\in F_1$;
        \end{itemize}
  \item $\forall (i,s)\in S,\ \forall (j,t)\in T.\ ((i,s),(j,t))\in I$ whenever either $i = j$ and $(s,t)\in I_i$
        or $i\neq j$; and
  \item $\forall (i,s)\in S.\ \mathsf{m}(i,s) = \mathsf{m}_i(s)$
 \end{itemize}
 is their \emph{product} and $(\pi^i_S, \pi^i_T) : \resarcn{V}{\bwdset{i}}{i} \to \resarcn{V}{\bwdset{0}}{0} + \resarcn{V}{\bwdset{1}}{1}$ defined as
 $(s,(i,s))\in \pi^i_S$ and $\pi^i_T(t) = (i,t)$ are the injections.
\end{prop}
\begin{proof}
 $\resarcn{V}{\bwdset{0}}{0} + \resarcn{V}{\bwdset{1}}{1}$ is clearly a \racn. It remains to prove that is indeed
 a coproduct in the category $\mathbf{RACN}$. 
\end{proof}


